Enhancing Federated Learning with Kolmogorov-Arnold Networks: A Comparative Study Across Diverse Aggregation Strategies

Multilayer Perceptron (MLP), as a simple yet powerful model, continues to be widely used in classification and regression tasks. However, traditional MLPs often struggle to efficiently capture nonlinear relationships in load data when dealing with complex datasets. Kolmogorov-Arnold Networks (KAN), inspired by the Kolmogorov-Arnold representation theorem, have shown promising capabilities in modeling complex nonlinear relationships. In this study, we explore the performance of KANs within federated learning (FL) frameworks and compare them to traditional Multilayer Perceptrons. Our experiments, conducted across four diverse datasets demonstrate that KANs consistently outperform MLPs in terms of accuracy, stability, and convergence efficiency. KANs exhibit remarkable robustness under varying client numbers and non-IID data distributions, maintaining superior performance even as client heterogeneity increases. Notably, KANs require fewer communication rounds to converge compared to MLPs, highlighting their efficiency in FL scenarios. Additionally, we evaluate multiple parameter aggregation strategies, with trimmed mean and FedProx emerging as the most effective for optimizing KAN performance. These findings establish KANs as a robust and scalable alternative to MLPs for federated learning tasks, paving the way for their application in decentralized and privacy-preserving environments.

==> figures.tex <==
\clearpage
\begin{figure*}[t]
    \centering
    \subfloat[\centering Best decision of Broker 1 under linear cost function \label{fig:1-1}]{{\includegraphics[width=0.25\textwidth]{Figures/1-1.png} }}
    \subfloat[\centering Best decision of Broker 2 under linear cost function \label{fig:1-2}]{{\includegraphics[width=0.25\textwidth]{Figures/1-2.png} }}
    \subfloat[\centering Utility of Broker 1 with linear cost function under different decision of two brokers \label{fig:1-3}]{{\includegraphics[width=0.25\textwidth]{Figures/1-3.png} }}
    \subfloat[\centering Utility of Broker 2 with linear cost function under different decision of two brokers \label{fig:1-4}]{{\includegraphics[width=0.25\textwidth]{Figures/1-4.png} }}
    \caption{Linear cost function}
    \label{figL}
\end{figure*}

\begin{figure*}[h]
    \centering
    \subfloat[\centering Best decision of Broker 1 under quadratic cost function \label{fig:2-1}]{{\includegraphics[width=0.25\textwidth]{Figures/2-1.png} }}%
    \subfloat[\centering Best decision of Broker 2 under quadratic cost function \label{fig:fig:2-2}]{{\includegraphics[width=0.25\textwidth]{Figures/2-2.png} }}%
    \subfloat[\centering Utility of Broker 1 with quadratic cost function under different decision of two brokers \label{fig:2-3}]{{\includegraphics[width=0.25\textwidth]{Figures/2-3.png} }}%
    \subfloat[\centering Utility of Broker 2 with linear quadratic function under different decision two both brokers \label{fig:fig:2-4}]{{\includegraphics[width=0.25\textwidth]{Figures/2-4.png} }}%
    \caption{Quadratic cost function}
    \label{figQ}
\end{figure*}

\begin{figure*}[h]
    \centering
    \subfloat[\centering Best decision of Broker 1 under exponential cost function \label{fig:3-1}]{{\includegraphics[width=0.25\textwidth]{Figures/3-1.png} }}%
    \subfloat[\centering Best decision of Broker 2 under exponential cost function \label{fig:3-2}]{{\includegraphics[width=0.25\textwidth]{Figures/3-2.png} }}%
    \subfloat[\centering Utility of Broker 1 with exponential function under different decision of two brokers \label{fig:3-3}]{{\includegraphics[width=0.25\textwidth]{Figures/3-3.png} }}%
    \subfloat[\centering Utility of Broker 2 with exponential function under different decision of two brokers \label{fig:3-4}]{{\includegraphics[width=0.25\textwidth]{Figures/3-4.png} }}%
    \caption{Exponential cost function}%
    \label{figE}%
\end{figure*}

\begin{figure*}[h]
    \centering
    \subfloat[\centering Best decision of Broker 1 under logarithmic cost function \label{fig:4-1}]{{\includegraphics[width=0.25\textwidth]{Figures/4-1.png} }}%
    \subfloat[\centering Best decision of Broker 2 under logarithmic cost function \label{fig:4-2}]{{\includegraphics[width=0.25\textwidth]{Figures/4-2.png} }}%
    \subfloat[\centering Utility of Broker 1 with logarithmic function under different decision of two brokers \label{fig:4-3}]{{\includegraphics[width=0.25\textwidth]{Figures/4-3.png} }}%
    \subfloat[\centering Utility of Broker 2 with logarithmic function under different decision of two brokers \label{fig:4-4}]{{\includegraphics[width=0.25\textwidth]{Figures/4-4.png} }}%
    \caption{Logarithmic cost function}%
    \label{figLOG}%
\end{figure*}
\clearpage
